Temperature-sensitive Soft Microgels at Interfaces: Air-Water versus Oil-Water

The formation of smart emulsions or foams whose stability can be controlled on-demand by switching external parameters is of great interest for basic research and applications. An emerging group of smart stabilizers are microgels, which are nano- and micro-sized, three-dimensional polymer networks that are swollen by a good solvent. In the last decades, the influence of various external stimuli on the two-dimensional phase behavior of microgels at air- and oil-water interfaces has been studied. However, the impact of the top-phase itself has been barely considered. Here, we present data that directly address the influence of the top-phase on the microgel properties at interfaces. The dimensions of pNIPAM microgels are measured after deposition from two interfaces, i.e., air- and decane-water. While the total in-plane size of the microgel increases with increasing interfacial tension, the portions or fractions of the microgels situated in the aqueous phase are not affected. We correlate the area microgels occupy to the surface tensions of the interfaces, which allows to estimate an elastic modulus. In comparison to nanoindentation measurements, we observe a larger elastic modulus for the microgels. By combining compression, deposition, and visualization, we show that the two-dimensional phase behavior of the microgel monolayers is not altered, although the microgels have a larger total in-plane size at higher interfacial tension. A peer reviewed and extended version of this preprint and the electronic supplementary information can be found under S.~Bochenek, A.~Scotti, W.~Richtering, \textit{Soft Matter}, 2020, DOI: 10.1039/d0sm01774d.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
